Neuro-symbolic Learning Yielding Logical Constraints

Neuro-symbolic systems combine the abilities of neural perception and logical reasoning. However, end-to-end learning of neuro-symbolic systems is still an unsolved challenge. This paper proposes a natural framework that fuses neural network training, symbol grounding, and logical constraint synthesis into a coherent and efficient end-to-end learning process. The capability of this framework comes from the improved interactions between the neural and the symbolic parts of the system in both the training and inference stages. Technically, to bridge the gap between the continuous neural network and the discrete logical constraint, we introduce a difference-of-convex programming technique to relax the logical constraints while maintaining their precision. We also employ cardinality constraints as the language for logical constraint learning and incorporate a trust region method to avoid the degeneracy of logical constraint in learning. Both theoretical analyses and empirical evaluations substantiate the effectiveness of the proposed framework.

==> contents/004_theory.tex <==
\section{Theoretical Analysis} \label{sec:theory}

 \section{Proof of Proposition 2}

 \begin{proof}
 \underline{\bf Notations.} We use $\|\cdot\|$ to denote the $\ell_2$ norm for vectors and Frobenius norm for matrices. 
 We define
 \begin{equation*}
 \varphi(\bm{\phi}, \bm{\theta}, \s{Z}, \s{Y}) := \|\s{Z} \m{w}_u + \s{Y} \m{w}_v - \m{b} \|^2 + \alpha \|(\s{Z}, \s{Y}) - (f_{\bm{\theta}}(\s{X}), \s{Y})\|^2, 
 \end{equation*}
 For short, we define $\Delta^k = f_{\m{\theta}^k}(\s{X})\m{w}_u^{k} + \s{Y} \m{w}_v^k - \m{b}$. 
 We also denote $\sigma_{\mathrm{min}}$ and $\sigma_{\mathrm{max}}$ as the smallest and largest non-zero eigenvalue of the covariance matrix $(f_{\bm{\theta}^k}(\s{X}); \s{Y})^{\tp}(f_{\bm{\theta}^k}(\s{X}), \s{Y})$, respectively. 
 Furthermore, by using the Woodbury identity formula, we can compute
 \begin{equation*}
 \begin{aligned}
 ({\s{Z}}^{k}; {\s{Y}}^{k})  & = {\arg\min}_{(\s{Z}, \s{Y})} \|\s{Z} \m{w}_u^k + \s{Y} \m{w}_v^k - \m{b} \|^2 + \alpha \|(\s{Z}, \s{Y}) - (f_{\bm{\theta}^k}(\s{X}), \s{Y})\|^2 \\
 % &  =  (\m{b} \m{w}^{\tp} + \alpha \s{Y} + \alpha f_{\bm{\theta}}(\s{X})) (\m{w} \m{w}^{\tp}+ \alpha \m{I})^{-1}. \\
 % &  = (\m{b} \m{w}^{\tp} + \alpha \s{Y} + \alpha f_{\bm{\theta}}(\s{X})) (\frac{1}{\alpha} \m{I} - \frac{1}{\alpha(\alpha+\m{w}^{\tp}\m{w})}\m{w}\m{w}^T) \\
 % &  = (f_{\m{\theta}^{k}}(\s{X}); \s{Y}) + \frac{(\m{b} - \s{Y} \m{w}^k - f_{\m{\theta}^k}(\s{X})\m{w}^{k})(\m{w}^{k})^{\tp}}{(\alpha+({\m{w}^{k}})^{\tp}\m{w}^{k})}  \\
 &  = (f_{\m{\theta}^{k}}(\s{X});\s{Y}) - \beta^k \Delta^k (\m{w}^{k})^{\tp}, 
 \quad \text{where} \quad \beta^k =\frac{1}{\alpha+ \|{\m{w}^{k}}\|^2}.
 \end{aligned}
 \end{equation*}
 %We also define
 %\begin{equation*}
 %\ell_1^k(\m{\theta}) = \varphi(\bm{\phi}^{k+1}, \bm{\theta}, \s{Z}^{k+1/2}, \s{Y}^{k+1/2}), \quad \ell_2(\m{\phi}) = \varphi(\bm{\phi}, \bm{\theta}^k, f_{\m{\theta}^k}(\s{X}), \s{Y}).
 %\end{equation*}
 Note that we also have 
 \begin{equation*}
 \begin{aligned}
 \varphi(\m{\phi}^k, \m{\theta}^k, \s{Z}^k,\s{Y}^k) &= (1- \beta^k (\m{w}^k)^{\tp}\m{w}^k)^2 \|\Delta^k\|^2 + (\beta^k (\m{w}^k)^{\tp}\m{w}^k)^2 \|\Delta^k\|^2 \\
 &= ((\alpha \beta^k)^2 + (1-\alpha \beta^k)^2) \|\Delta^k\|^2 \ge \frac{\rho}{\rho+1} \|\Delta^k\|^2, \quad \rho > 1.
 \end{aligned}
 \end{equation*}
 Hence
 \begin{equation*}
 \begin{aligned}
  \varphi(\m{\phi}^k, \m{\theta}^k, f_{\m{\theta}^k}(\s{X}), \s{Y}) -  \varphi(\m{\phi}^k, \m{\theta}^k, \s{Z}^k, \s{Y}^k) = (1 - (\alpha \beta^k)^2 - (1-\alpha \beta^k)^2) \|\Delta^k\|^2.
  \end{aligned}
 \end{equation*}

 \underline{\bf Update of $\m{\phi}$}. 
 For simplicity, we consider the single rule case (multiple rules can be directly decomposed), i.e., $\m{\phi} = (\m{w}, \m{b})$ and $\m{b} = (b; \dots; b)$. 
 The update of $\m{\phi}$ is conducted on the loss function 
 \begin{equation*}
 \ell_2^k(\m{w}, \m{b}) = \varphi(\m{\phi}^k, \m{\theta}^k, f_{\m{\theta}^k}(\s{X}), \s{Y})  = \|f_{\m{\theta}^k}(\s{X}) \m{w}_u + \s{Y} \m{w}_v - \m{b} \|^2. 
 \end{equation*}
 We update $b$ by $b = \frac{1}{N} \sum_{i=1}^N [f_{\m{\theta}^k}(\s{X})\m{w}_u^{k} + \s{Y} \m{w}_v^k]_i$, 
 and update $\m{w}$ by PPA method, i.e.,
 \begin{equation*}
 \m{w}^{k+1} = \arg\min_{\m{w}} \ell_2^k(\m{w}, \m{b}) + \frac{1}{\gamma} \|\m{w} - \m{w}^k\|^2, 
 \end{equation*}
 which can be reduced to
 \begin{equation*}
 \m{w}^{k+1} - \m{w}^k = - \m{M}^{k} \m{\delta}^k, \quad \m{\delta}^k =  (f_{\bm{\theta}^k}(\s{X}), \s{Y})^{\tp} \Delta = \nabla_{\m{w}} \ell_2^k(\m{w}, \m{b}),
 \end{equation*}
 where
 \begin{equation*}
 \m{M}^k=\big((f_{\bm{\theta}^k}(\s{X}), \s{Y})^{\tp}(f_{\bm{\theta}^k}(\s{X}), \s{Y}) + \epsilon \m{I}\big)^{-1}, \quad \epsilon = 1/\gamma.
 \end{equation*} 
 
 By using the $(2/\gamma)$-strongly convexity of the proximal term, we obtain that
 \begin{equation*}
 \begin{aligned}
 \varphi(\m{\phi}^{k}, \m{\theta}^{k}, \s{Z}^{k}, \s{Y}^k) &  =  \varphi(\m{\phi}^k, \m{\theta}^k, f_{\m{\theta}^k}(\s{X}), \s{Y}) - (1 - (\alpha \beta^k)^2 - (1-\alpha \beta^k)^2) \|\Delta\|^2 \\
 & = \ell_2^k(\m{w}^k, \m{b}) -  (1 - (\alpha \beta^k)^2 - (1-\alpha \beta^k)^2) \|\Delta\|^2 \\
 & \ge \ell_2^k(\m{w}^{k+1}, \m{b}) - (1 - (\alpha \beta^k)^2 - (1-\alpha \beta^k)^2) \|\Delta\|^2 + \frac{2}{\gamma}\|\m{w}^{k+1}-\m{w}^k\|^2. 
 \end{aligned}
 \end{equation*}
 Plugging $\m{w}^{k+1}-\m{w}^k = - \m{M}^k\m{\delta}^k$ into the inequality, we have
 %\begin{equation*}
 %\begin{aligned}
 %\langle \nabla_{\m{w}} \ell_2^k(\m{w}^k, \m{b}), \m{w}^{k+1} - \m{w}^k \rangle &= 2 (\Delta^k)^{\tp} (f_{\m{\theta}^k}(\s{X}), \s{Y}) (\m{w}^{k+1} - \m{w}^k)  = 2(\m{\delta}^k^k)^{\tp} \m{M}^k \m{\delta}^k.
 %\end{aligned}
 %\end{equation*}
 %Now, with $\gamma \leq 1/\sigma_{\max}$, we have 
 \begin{equation*} 
 \begin{aligned}
  \varphi(\m{\phi}^{k}, \m{\theta}^{k}, \s{Z}^{k}, \s{Y}^k)  & \ge \ell_2^k(\m{w}^{k+1}, \m{b})  - (1 - (\alpha \beta^k)^2 - (1-\alpha \beta^k)^2) \|\Delta\|^2 +  \frac{2}{\gamma}  (\m{\delta}^k)^{\tp} (\m{M}^k)^2 \m{\delta}^k \\
 & \ge \varphi(\m{\phi}^{k+1}, \m{\theta}^{k}, \s{Z}^{k+1/2}, \s{Y}^{k+1/2}) + \frac{2}{\gamma} (\m{\delta}^k)^{\tp} (\m{M}^k)^2 \m{\delta}^k  -  \frac{1}{\rho+1} \|\Delta\|^2,
 \end{aligned}
 \end{equation*}
 %Next, we construct the gap between $\ell_2^k(\m{w}^{k+1}, \m{b})$ and $\varphi(\m{\phi}^{k+1}, \m{\theta}^{k}, \s{Z}^{k+1/2}, \s{Y}^{k+1/2})$, 
 where
 \begin{equation*}
 \begin{aligned}
  & ({\s{Z}}^{k+1/2}; {\s{Y}}^{k+1/2})  = {\arg\min}_{(\bar{\s{Z}}, \bar{\s{Y}})} \|\bar{\s{Z}} \m{w}_u^{k+1} + \bar{\s{Y}} \m{w}_v^{k+1} - \m{b} \|^2 + \alpha \|(\bar{\s{Z}}, \bar{\s{Y}}) - (f_{\bm{\theta}^k}(\s{X}), \s{Y})\|^2 \\
 & \qquad \qquad  = (f_{\m{\theta}^{k}}(\s{X});\s{Y}) - \beta^{k+1/2} \Delta^{k+1/2} (\m{w}^{k+1})^{\tp}, 
 \quad \text{where} \quad \beta^{k+1/2} =\frac{1}{\alpha+\|{\m{w}^{k+1}}\|^2}.
 \end{aligned}
 \end{equation*}
 %Using ($2\alpha$)-strongly convexity of $\varphi$ in $(\s{Z}, \s{Y})$ and the Cauchy–Schwarz inequality, we have
 %\begin{equation*}
 %\begin{aligned}
 %& \ell_2^k(\m{w}^{k+1}, \m{b}) - \varphi(\m{\phi}^{k+1}, \m{\theta}^{k}, \s{Z}^{k+1/2}, \s{Y}^{k+1/2}) - \frac{1}{\alpha} \|\Delta^k (\m{w}^k)^{\tp}\|^2 \\
 %& \qquad \qquad \qquad \qquad  = \varphi(\m{\phi}^{k+1}, \m{\theta}^k, f_{\m{\theta}^k}(\s{X}), \s{Y}) -  \varphi(\m{\phi}^{k+1}, \m{\theta}^k, \s{Z}^{k+1/2}, \s{Y}^{k+1/2}) - \frac{1}{\alpha} \|\Delta^k (\m{w}^k)^{\tp}\|^2 \\
 % & \qquad \qquad \qquad \qquad \ge \alpha \| \beta^{k} \Delta^{k} (\m{w}^{k})^{\tp} - \beta^{k+1/2} \Delta^{k+1/2} (\m{w}^{k+1})^{\tp}\|^2 - \frac{1}{\alpha} \|\Delta^k (\m{w}^k)^{\tp}\|^2 \\
 % \end{aligned}
 %\end{equation*}
 The last term $\m{\delta}^k (\m{M}^k)^2 \m{\delta}^k$ can be computed as
 \begin{equation*}
 \begin{aligned}
 \m{\delta}^k (\m{M}^k)^2 \m{\delta}^k = (\Delta^k)^{\tp}  (f_{\bm{\theta}^k}(\s{X}), \s{Y}) (\m{M}^k)^2  (f_{\bm{\theta}^k}(\s{X}), \s{Y})^{\tp} \Delta^k 
 \end{aligned}
 \end{equation*}
 If $\|\m{\delta}^k\| \neq 0$, we can know that $\Delta^k$ is in the row space of $(f_{\bm{\theta}^k}(\s{X}),\s{Y})$, and thus we have
 \begin{equation*}
 \frac{2}{\gamma} \m{\delta}^k (\m{M}^k)^2 \m{\delta}^k \ge \min(\kappa_1, \kappa_2) \|\Delta\|^2, \quad \text{where} \quad \kappa_1 =  \frac{2\gamma \sigma_{\max}}{(1+\gamma \sigma_{\max})^2}, \quad \kappa_2 = \frac{2\gamma \sigma_{\min}}{(1+\gamma \sigma_{\min})^2}. 
 \end{equation*}
 To ensure $\min(\kappa_1, \kappa_2) > \frac{1}{\rho+1}$, we set the stepsize $\gamma$ to
 \begin{equation*}
 \begin{aligned}
 \gamma \in  [\frac{\rho-(\rho^2-1)^{\frac{1}{2}}}{\sigma_{\max}}, \frac{\rho+(\rho^2-1)^{\frac{1}{2}}}{\sigma_{\max}}],  \quad \text{and} \quad \gamma \in  [\frac{\rho-(\rho^2-1)^{\frac{1}{2}}}{\sigma_{\min}}, \frac{\rho+(\rho^2-1)^{\frac{1}{2}}}{\sigma_{\min}}], 
 \end{aligned}
 \end{equation*}
 for cases $\kappa_1 < \kappa_2$ and $\kappa_1 > \kappa_2$, respectively. 
 Hence, there exists a positive constant $c>0$ such that
 \begin{equation*}
 \frac{2}{\gamma} \m{\delta}^k (\m{M}^k)^2 \m{\delta}^k -  \frac{1}{\rho+1} \|\Delta\|^2 \ge c \m{\delta}^k (\m{M}^k)^2 \m{\delta}^k \ge \frac{c\gamma}{1+\gamma \sigma_{\max}} \|\m{\delta}\|^2
 \end{equation*}
 Putting together, we obtain that
 \begin{equation*}
 \varphi(\m{\phi}^{k}, \m{\theta}^{k}, \s{Z}^{k}, \s{Y}^{k}) \ge \varphi(\m{\phi}^{k+1}, \m{\theta}^{k}, \s{Z}^{k+1/2}, \s{Y}^{1+1/2}) + \frac{c\gamma}{1+\gamma \sigma_{\max}} \|\nabla_{\m{\phi}} \ell_2(\m{w}, \m{b})\|^2
 \end{equation*}

 \underline{\bf Update of $\m{\theta}$}. 
 The update of $\m{\theta}$ is conducted on the loss function
 \begin{equation*}
 \ell_2^k(\m{\theta}) = \|\s{Z}^{k+1/2} - f_{\m{\theta}}(\s{X})\|^2. 
 \end{equation*}
 By using $\mu_{\m{\theta}}$-smooth of $\ell_1^k$, we obtain that 
 \begin{equation*}
 \begin{aligned}
 & \varphi(\m{\phi}^{k+1}, \m{\theta}^{k}, \s{Z}^{k+1/2}, \s{Y}^{k+1/2}) - \varphi(\m{\phi}^{k+1}, \m{\theta}^{k+1}, \s{Z}^{k+1/2}, \s{Y}^{k+1/2}) = \ell_2^k(\m{\theta}^{k+1}) - \ell_2^k(\m{\theta}^k) \\
  & \quad \qquad \qquad \qquad \qquad  \ge  - \langle \nabla_{\m{\theta}} \ell_2^k(\m{\theta}^k), \m{\theta}^{k+1} - \m{\theta}^k \rangle - \frac{\mu_{\theta}}{2} \|\m{\theta}^{k+1} - \m{\theta}^k\|^2  \ge \frac{1}{2} \eta \|\nabla_{\m{\theta}} \ell_2^k(\m{\theta}^k)\|^2. 
 \end{aligned}
 \end{equation*}
 Letting $\s{Z}^{k+1} = {\arg\min}_{\s{Z}} ~\varphi(\bm{\phi}^{k+1}, \bm{\theta}^{k+1}, {\s{Z}})$, 
 we conclude
 \begin{equation*}
 \begin{aligned}
 \varphi(\m{\phi}^{k+1}, \m{\theta}^k, \s{Z}^{k+1/2}, \s{Y}^{k+1/2})  \ge \varphi(\m{\phi}^{k+1}, \m{\theta}^{k+1}, \s{Z}^{k+1}, \s{Y}^{k+1}) + \frac{1}{2} \eta \|\nabla_{\m{\theta}} \ell_2^k(\m{\theta}^k)\|^2. 
 \end{aligned}
 \end{equation*}

 \underline{\bf Convergent result.} 
 By combining the update of $\m{\phi}$ and $\m{\theta}$, we have
 \begin{equation*}
 \begin{aligned}
 & \varphi(\m{\phi}^{k}, \m{\theta}^k, \s{Z}^k, \s{Y}^k) - \varphi(\m{\phi}^{k+1}, \m{\theta}^{k+1}, \s{Z}^{k+1}, \s{Y}^{k+1}) \\
 & \qquad \qquad \qquad \qquad \qquad \qquad \ge \frac{1}{2} \eta \|\nabla_{\m{\theta}} \ell_2^k(\m{\theta}^k)\|^2 + \frac{c\gamma}{1+\gamma \sigma_{\max}} \|\nabla_{\m{\phi}} \ell_2(\m{w}, \m{b})\|^2. 
 \end{aligned}
 \end{equation*}
 Taking a telescopic sum over $k$, we obtain
 \begin{equation*}
 \begin{aligned}
 & \varphi(\m{\phi}^{0}, \m{\theta}^0, \s{Z}^0, \s{Y}^0)  - \varphi(\m{\phi}^{K}, \m{\theta}^{K}, \s{Z}^{K}, \s{Y}^K) \\
 & \qquad \qquad \qquad \qquad \qquad \qquad \ge \sum_{i=1}^K \frac{1}{2} \eta \|\nabla_{\m{\theta}} \ell_2^k(\m{\theta}^k)\|^2 + \frac{c\gamma}{1+\gamma \sigma_{\max}} \|\nabla_{\m{\phi}} \ell_2(\m{w}, \m{b})\|^2. 
 \end{aligned}
 \end{equation*}
 Hence, we have
 \begin{equation*}
 \mathbb{E}[\|\nabla_{\m{\theta}} \ell_2^k(\m{\theta}^k)\|^2] \leq  \frac{2}{K\eta}\big(\varphi(\m{\phi}^{0}, \m{\theta}^0, \s{Z}^0, \s{Y}^0) - \min  \varphi(\m{\phi}, \m{\theta}, \s{Z}, \s{Y})\big),
 \end{equation*}
 and
 \begin{equation*}
 \mathbb{E}[\|\nabla_{\m{\phi}} \ell_2(\m{w}, \m{b})\|^2] \leq  \frac{1+\gamma\sigma_{\max}}{Kc\gamma}\big(\varphi(\m{\phi}^{0}, \m{\theta}^0, \s{Z}^0, \s{Y}^0) - \min  \varphi(\m{\phi}, \m{\theta}, \s{Z}, \s{Y})\big). 
 \end{equation*}
 \end{proof}
% \input{contents/004_theory}





==> contents/007_preliminary.tex <==
\section{Preliminary} \label{sec: preliminary}

==> slides/beamer/fig1.tex <==
\tikzstyle{vertex}=[circle,fill=black!25,minimum size=20pt,inner sep=0pt]
\tikzstyle{selected vertex} = [vertex, fill=red!24]
\tikzstyle{edge} = [draw,thick,-]
\tikzstyle{weight} = [font=\small]
\tikzstyle{selected edge} = [draw,line width=3pt,-,red!50]
\tikzstyle{ignored edge} = [draw,line width=3pt,-,black!20]

\begin{figure}
\begin{tikzpicture}[scale=0.6, auto,swap]
  \tikzstyle{every node}=[scale=0.6]
    % Draw a 7,11 network
    % First we draw the vertices
    \foreach \pos/\name in {{(0,2)/a}, {(2,1)/b}, {(4,1)/c},
                            {(0,0)/d}, {(3,0)/e}, {(2,-1)/f}, {(4,-1)/g}}
        \node[vertex] (\name) at \pos {$\name$};
    % Connect vertices with edges and draw weights
    \foreach \source/ \dest /\weight / \pos in {b/a/2/above, c/b/8/above,d/a/3/left,d/b/9/above,
                                         e/b/1/right, e/c/2/left,e/d/15/above,
                                         f/d/1/above,f/e/9/left,
                                         g/e/9/left,g/f/11/below}
        \path[edge] (\source) -- node[\pos, weight] {$\weight$} (\dest);
%    % Start animating the vertex and edge selection. 
     \foreach \vertex / \fr in {d/1,a/2,f/3,b/4,e/5, c/6} % ,c/6,g/7}
         \path node[selected vertex] at (\vertex) {$\vertex$};
%    % For convenience we use a background layer to highlight edges
%    % This way we don't have to worry about the highlighting covering
%    % weight labels. 
   \begin{pgfonlayer}{background}
        \foreach \source / \dest in {d/a,d/f,a/b,b/e,e/c}
            \path[selected edge] (\source.center) -- (\dest.center);
        \foreach \source / \dest / \fr in {d/b/4,d/e/5,e/f/5,b/c/6,f/g/7, e/g/8}
            \path[ignored edge] (\source.center) -- (\dest.center);
    \end{pgfonlayer}
\end{tikzpicture}
\caption{Compute the shortest path. \\
$d(c, f) = d(f, a) + d(a, c)$.}
\end{figure}


